High performance single-photon sources at telecom wavelength based on broadband hybrid circular Bragg gratings

Semiconductor quantum dots embedded in hybrid circular Bragg gratings are a promising platform for the efficient generation of nonclassical light. The scalable fabrication of multiple devices with similar performance is highly desirable for their practical use as sources of single and entangled photons, while the ability to operate at telecom wavelength is essential for their integration with the existing fiber infrastructure. In this work we combine the promising properties of broadband hybrid circular Bragg gratings with a membrane-transfer process performed on 3" wafer scale. We develop and study single-photon sources based on InAs/GaAs quantum dots emitting in the telecom O-band, demonstrating bright single-photon emission with Purcell factor > 5 and count rates up to 10 MHz. Furthermore, we address the question of reproducibility by benchmarking the performance of 10 devices covering a wide spectral range of 50 nm within the O-band.

==> Section_5/Section_5.tex <==
\section{Conclusions}
%
%
\noindent In summary,
